Understanding Deep Networks via Extremal Perturbations and Smooth Masks

The problem of attribution is concerned with identifying the parts of an input that are responsible for a model's output. An important family of attribution methods is based on measuring the effect of perturbations applied to the input. In this paper, we discuss some of the shortcomings of existing approaches to perturbation analysis and address them by introducing the concept of extremal perturbations, which are theoretically grounded and interpretable. We also introduce a number of technical innovations to compute extremal perturbations, including a new area constraint and a parametric family of smooth perturbations, which allow us to remove all tunable hyper-parameters from the optimization problem. We analyze the effect of perturbations as a function of their area, demonstrating excellent sensitivity to the spatial properties of the deep neural network under stimulation. We also extend perturbation analysis to the intermediate layers of a network. This application allows us to identify the salient channels necessary for classification, which, when visualized using feature inversion, can be used to elucidate model behavior. Lastly, we introduce TorchRay, an interpretability library built on PyTorch.

==> fig-area-norm.tex <==
\begin{figure}
\centering
\includegraphics[width=0.8\linewidth]{area_loss.pdf}
\caption{\textbf{Area constraint.}
The blue line is the reference vector $\mathbf{r}_a$ representing the target area $a$ as a proportion of ``on'' versus ``off'' pixels (here $a=80\%$).
The red dotted lines represent mask values in ascending, sorted order, $\sortvec(\bbm)$, at different points of the optimization, staring by initializing $\bbm$ to $1/2$.
Over time, the optimization encourages the mask to match the target area.
Even in the limit, there is a slight difference between  $\mathbf{r}_a$ as $\bbm$ as the latter is forced to be smooth at the boundaries; this has the further beneficial effect of minimizing the boundary length, encouraging more compact masks.
}\label{fig:area_norm}
\end{figure}


==> fig-correlation-compactness.tex <==
\begin{figure}
\centering
\includegraphics[width=0.49\linewidth]{mean_channels_hist.pdf}
\caption{\textbf{Compactness.} Left: This plot shows that the mean, minimally sufficient area for channel-wise perturbation masks for a class is typically less than 75 channels. }
\label{fig:correlation_compactness}
\end{figure}

==> fig-cppn-channel.tex <==
\begin{figure}
\centering
\includegraphics[width=0.32\linewidth]{cppn_channel_162_class_dalmatian_251.pdf}
\includegraphics[width=0.32\linewidth]{cppn_channel_166_class_hamster_333.pdf}
\includegraphics[width=0.32\linewidth]{cppn_channel_723_class_damselfly_320.pdf}
\includegraphics[width=0.32\linewidth]{cppn_channel_747_class_drilling_platform_540.pdf}
\includegraphics[width=0.32\linewidth]{cppn_channel_806_class_gondola_576.pdf}
\includegraphics[width=0.32\linewidth]{cppn_channel_810_class_canoe_472.pdf}
\caption{\textbf{Discovery of Class-Specific Channels.} By analyzing the channel-wise masks, we automatically find these highly class-specific channels. Each of these channels were included in the extremal, channel-wise masks of all 50 ImageNet validation images of a class (18 channels fit this criteria; rightmost part   of~\cref{fig:correlation_compactness}b). We use Compositional Pattern Producing Networks (CPPNs)~\cite{mordvintsev2018differentiable, stanley2007compositional} to generate these inversions.}
\label{fig:cppn_channel}
\end{figure}

==> fig-mask-generation.tex <==
\begin{figure}
\centering
\includegraphics[width=\linewidth]{mask_generation.pdf}
\caption{\textbf{Generating smooth masks.}
a. We first define a low resolution parameterization mask, $\bar\bbm \in [0,1]^{H \times W}$ (shown as a binary mask in this illustration).
b. We then represent each location in $\bar \bbm$ as a high resolution, smooth Gaussian, weighted by the value in $\bar\bbm$.
c. Finally, we apply the smooth max operator $...$ across all locations to get our final mask.}\label{fig:mask_generation}
\end{figure}

==> fig-pointing-examples.tex <==
\begin{figure}
\centering
\includegraphics[width=0.3\linewidth]{000025_class_cow_9.pdf}
\includegraphics[width=0.3\linewidth]{000058_class_person_14.pdf}
\includegraphics[width=0.3\linewidth]{000069_class_boat_3.pdf}
\includegraphics[width=0.3\linewidth]{000025_class_person_14.pdf}
\includegraphics[width=0.3\linewidth]{000058_class_motorbike_13.pdf}
\includegraphics[width=0.3\linewidth]{000069_class_person_14.pdf}
\caption{\textbf{Pointing Examples from PASCAL}. Here we see a few examples of where our method is able to localize well to different objects in the image. The overlaid visualization is the average mask after Gaussian smoothing ($\sigma = 20$).}\label{fig:pointing-examples}
\end{figure}

==> scratch.tex <==
\begin{equation*}
\label{e:extremal_perturbation}
\arraycolsep=2pt
\begin{array}{lcl}
\forall \bx : |\bx' - \bx| < \delta
&\Rightarrow&
\Big|
\Phi(\bx') - \langle \nabla \Phi(\bx), \bx' - \bx \rangle - \Phi(\bx)
\Big| < \epsilon,\\
\forall \bbm : |\bbm| < a^*
&\Rightarrow&
\Phi(\bbm \otimes \bx) < \Phi(\bx).\\
\end{array}
\end{equation*}

\subsection{Old intro}

Machine learning allows to build models with excellent empirical performance in many applications.
However, the resulting models, which are extracted automatically from data, are rather opaque and of difficult characterization.
In particular, it is difficult to say what knowledge they embody and what are their limitations.
Answering these questions is important from a technical perspective, but also to ensure that models are adequate in applications where safety or fairness are important.

Several authors have thus looked at the problem of characterizing the properties of learned models.
These are regarded as given functions $\Phi : \mathcal{X} \rightarrow \mathbb{R}^d$ mapping data $x\in\mathcal{X}$ to labels or representation vectors $\Phi(x)$.
The goal is to ``explain''  what such a function ``does''.
For example, if the output of the function $\Phi(x)$ is highly correlated with a \emph{cat} being contained in the image, we may say that the function recognizes cats.

The space of possible explanations is of course very large, and the challenge is to find out explanations that are insightful and useful.
In this paper, we improve and generalize three popular explanation techniques.
We start by the concept of \emph{meaningful perturbations}, namely applying informative transformations $tx$ to an image $x$ so as to probe the effect of such changes on the output of the function $\Phi(tx)$.
In~\cite{fong17interpretable}, meaningful perturbations were introduced as a mean to address the question of attribution, namely identifying which parts in a particular image are responsible for the output of a deep neural networks.

Here we propose a number of improvements.
First, we ground formally the concept of \emph{extremal perturbation}, providing a better foundation for the explanations proposed by~\cite{fong17interpretable}.

Second, we revisit the issue of generating meaningful perturbations via punching holes or blurring parts of the image, creating a significant deviation from ``natural'' stimuli that are normally observed by the model.
We compare these techniques with: 1) training a network that observes perturbations during training and is thus less disrupted by it and 2) using the~\emph{deep image prior}~\cite{ulyanov18deep} to infill the image with a seamless and yet unbiased inpaint.

Third, we generalize input perturbations to perturbations applied to the intermediate layers of a deep neural networks.
We show that it is easier to blocking channel activations than perturbing the input image directly.
We also show that intermediate blocking can still be visualized in an intuitive and interpretable manner in the input image domain via \emph{partial inversion}, in which we extend the technique of~\cite{mahendran15understanding} to reconstruct only non-blocked activations.
This can be interpreted as a generalize version of punching holes where information rather than spatial locations are suppressed.

Finally, we look at the locality of the explanations.
In particular, we suggest a formal link between perturbation analysis and global analysis via externally labelled image semantics.
Based on this link, we then demonstrate running perturbation analysis in a global sense, studying the behavior of a network not on a single input stimulus, but across all possible ones.


\subsection{Explanation locality}

The most simple explanation is perhaps a single input-output pair $(x,f(x))$ showing what value the function $f$ takes on a point $x$. The explanatory power of a single pair is low, unless it is used to disprove a general claim. For example, $(x,f(x))$ where $x$ contains a cat and $f(x)$ is low is a \emph{counter example} to the claim that $f(x)$ is a cat classifier --- although all it would show is a single mistake that the classifier makes.

As humans, we are

In perturbation analysis we seek how the function $\Phi(x)$ changes as the input $x$ is changed (perturbed) in some interesting way.


In the simples case, we consider two samples $x$ and $x'$ related in a meaningful way and we compare the values of $\Phi(x)$ and $\Phi(x')$. Consider two examples:

1. If $x,x'$ are images related by a 45 degrees rotation, then a rotation-invariant representation would have $\Phi(x)=\Phi(x')$.

2. If $x$ contains a "cat",  $x'$ is the same image with the cat "deleted" and $\Phi(x)\in\mathbb{R}$ is the score of a "cat classifier", then we may expect $\Phi(x) \gg \Phi(x')$.

Formally, the explanation is the tuple

$$
   (x, x', \Phi(x), \Phi(x')).
$$

This is very little information. We may be *tempted* to think that 1. suggests that the representation is invariant to rotations and that 2. the classifier looks for the region in the image that contains a cat. However, the tuple is clearly insufficient to establish either facts.

Extremal perturbation

A more informative approach is to look for perturbations that are "extremal" in some sense. For instance, let $x'=dx$ be a version of $x$ after deleting a region and let $|d|$ be the size of the deleted region. Then we can seek for the *smallest* perturbation that causes a sufficiently large variation in the output $\Phi(dx)$:

$$
   d^* = \arg\min |d|,\quad \text{s.t.\ }
   \frac{\Phi(dx)}{\Phi(x)} < 0.01,
$$

where, assuming $\Phi(dx)\in\mathbb{R}_+$, we seek for the smallest deletion that causes a 99%

$$
 \forall d : |d| < |d^*| :
 \quad
 \frac{\Phi(dx)}{\Phi(x)} \geq 0.01.
$$

This approach thus fixes a point $x$ and looks at how "stable" the network $\Phi$ is around that point, where stability is measured in terms of magnitude of input perturbation.

This is the same as our ICCV paper on perturbation analysis.

Limitations:

- Perturbations can be artefacts: they cause a disproportionate effect to the value of the function by exploiting some quirk or singularity of its behaviour. These "adversarial" perturbations are *not* representative of the statistically significant behaviour of the function when applied to real data, but can significantly distort analysis by looking for extremal perturbations. This can be addressed by regularizing the perturbations $d$ (in the example above punishing such quirky deletions with a large norm $|d|$), but it is a hack.


Systematic perturbations

 An alternative approach is to fix a perturbation $g : \mathcal{X} \rightarrow \mathcal{X}$ and look at how systematic the response of $\Phi$ is to the effect of $g$ on data.

For example, if $g$ is an image rotation of 45 degrees, we can check for invariance

$$
 \forall x \in \mathcal{X}:
 \quad
 \Phi(x) = \Phi(gx)
$$

or, more in general, equivariance

$$
 \forall x \in \mathcal{X}:
 \quad
  M_g\Phi(x) = \Phi(gx)
$$

where $M_g$ is a mapping that reproduces the effect of $g$ directly in representation space. We have done a lot of work in the past that follows this idea with Karel Lenc.

More in general we can look for systematic behaviour for for all $x \in \mathcal{X}$ and $g \in G$:

$$
 \forall x \in \mathcal{X},\quad g\in G:
 \quad
  M_g\Phi(x) = \Phi(gx).
$$

LIME-like explanations

LIME seeks for an "interpretable" function $\eta(x)$ (often a linear function $Ax$) that approximates the function $\Phi(x)$, often limited to a neighbourhood $N(x_0)$ of a sample $x_0\in\mathcal{X}$. If the approximation is good, the explanation is said to be *faithful*:

$$
\forall x \in N(x_0): \quad
\Phi(x) \approx \eta(x).
$$

Given data samples, the explanation $A$ can then be fitted to the function $\Phi$ using machine learning methods.

LIME limitations:

- It is not obvious how to define the approximation function $\eta$ so that it is interpretable. A linear classifier defined on the pixels of an image $x$ may give us a notion of "saliency", but little more.

- The function $\eta$ may not be faithful, especially if it is simple enough to be interpretable. For example, neural networks defined on images are generally badly approximated by linear classifiers; as a consequence, the resulting "saliency" maps may not be very informative.

- The explanation is local in two ways: it explains a *single* network around a *single* data point $x$. Hence we may be able to know that a certain image region is important to detect a cat in an image, and that region may correspond to the cat. But we cannot know that the network looks for cats *in general*. We also do not know if looking at cat regions is important for all networks that are able to recognize such objects.

- Going back to the adequacy of linear approximations, first order pixel derivatives correspond to changes in an image (tweaking a single pixel) that are insufficient to observe a meaningful change in the neural network output $\Phi(x)$. More meaningful perturbation alter the image in a more substantial way (for example by deleting an entire image region).

Global-local LIME

An issue with LIME is not only that it looks for *local perturbations*, but that it does so around a single sample $x_0$. A variant is to learn an approximation function $\eta : \mathcal{X}\times\mathcal{X}\rightarrow \mathbb{R}^d$ that does so for all reference points $x_0$:

$$
\forall x_0\in\mathcal{X}:
\quad
\forall x\in N(x_0):
\quad
\Phi(x) \approx \eta(x|x_0).
$$

In other words, the approximation still describe the effect of local perturbations, but it does so for all input points, therefore capturing some information about the global structure of $\Phi$.

LIME vs perturbation analysis

In LIME we seek an approximation of the type:

$$
\forall x \in N(x_0): \quad
\eta(x) \approx \Phi(x).
$$

In systematic perturbation analysis we seek for an approximation of the type:

$$
\forall x \in \mathcal{X},\quad \forall g\in G:
\quad
M_g \Phi(x) \approx \Phi(gx)
$$

With slight abuse of notation, the latter reduces to LIME if $\mathcal{X} = \{x_0\}$,  $g(x_0) = x_0 + g$ and $G = N(x_0) - x_0$. In this case $\eta(x) = M_{x-x_0} \Phi(x_0)$.

In other words, LIME is a limited version of perturbation analysis in which one seeks for an approximation only around a specific point $x_0$ and in such a way that perturbations are characterized in a trivial manner (just as point in a neighbourhood of $x_0$). On the other hand, in perturbation analysis we want to characterise the response of the function $\Phi(x)$ to a *structured* perturbation (expressed by a transformation $g$) in a manner that applies to the whole input domain $\mathcal{X}$.

Explanations using data annotations

In perturbation analysis we must choose the perturbations $G$ a-priori. There aren't so many interesting choices here. For images, a typical one is to study invariance or equivariance to effects such as perspective distortion. 

All such effects are *independent* of the image content, whereas we would expect representation to be very sensitive to the content of the image.

Suppose now that, in addition to the data $x$, we are also given labels $y$. These may be the same labels used to train the network, or entirely different labels.

A typical approach in vision is to annotate lots of concepts in images and then check wether any neuron has learned any of such concept by looking for high correlations between neuron response $\Phi(x)$ and concept presence (as marked in $y$).

Correlating features and annotations by learning predictors

The easiest way to seek for these correlations is to look for a predictor $\Phi$ that maps $\Phi(x)$ to $y$:

$$
 \forall (x,y):
 \quad
 \Psi \circ \Phi(x) = y.
$$

In practice $\Psi$ is often a linear function; furthermore, we often look for a direct correlation between concepts in $y$ (seen as a 01-vector of possible concepts in an image, such as "cat", "red", "grass", "thin") and features $\Psi(x)$, so $\Psi$ is little more than a "permutation" matrix that associates feature dimensions to concepts.

The simpler $\Psi$ is, the more directly $\Phi(x)$ and $y$ are "correlated".

New Variants

Recall that perturbation analysis uses content-agnostic transformations $G$. If annotations are available, we can do content-aware perturbation analysis. For example, suppose that $y$ the bounding box of a "cat" in an image (if any) and $D_\mathcal{Y}$ a deletion of that image region. Now we can predict the effect of deleting such a region from a "cat" image; the simplest predictor is just an average percentage drop in classification score:

$$
E_{(x,y)}\left[ \frac{\Phi(D_\mathcal{Y}x)}{\Phi(x)} \right]
$$

A slight more sophisticated approach is to build an annotation-driven variant of LIME:

$$
    \forall (x_0,y_0):
    \quad
    \forall x \in N(x_0,y_0):
    \quad
    \eta(x|y_0) \approx \Phi(x).
$$

This is the same as global-local version of LIME above, except that the approximator uses $y_0$ rather than $x_0$. If this works, it means that the local behaviour of the function $\Phi(x)$ can be (at least in part) predicted by knowing the content of the image.

We can further play with the type of information used by the approximator $\eta$ as well as which information is "fixed" (so that a new approximator has to be learned if that part changes):


Note that in the last two examples we allow the approximator to work on top of the representation computed for $\Phi(x_0)$. This means that we are learning a **relationship between representations** as opposed to predict the representation directly (this is why we call this equivariance).

\newpage\cleardoublepage

\section{Method}\label{s:method}

We would like to ``explain'' a given function $\Phi : \mathcal{X} \rightarrow \mathbb{R}^d$ mapping data $x\in\mathcal{X}$ to code vectors $\Phi(x)$.
As in the case of deep neural networks, we usually have a concrete definition of the function, as well as a way of computing it, but not necessarily a good understanding of its properties.
An explanation is a compact and interpretable characterization of the properties of the function.
For example, we may say that the function $\Phi(x)$ recognizes ``cats'' if its output is highly correlated with cats being contained in images.

There is of course as many explanations as ways of characterizing a function, but only very few are useful.
Next, we review some ideas presented in the literature, unifying and polishing some of them, and then discuss extensions.

\subsection{Explanations using example input data}

We start by discussing types of explanations that only make use of an example set of input points $x\in\mathcal{X}$.

\paragraph{Differential perturbations.}

A standard analysis technique~\cite{simonyan14deep,ribeiro16why-should,selvaraju17grad-cam:} for deep neural networks is \emph{attribution},
namely identifying which components of the input $x$ contribute the most to determining the output $\Phi(x)$ of the function.

In computer vision, attribution is often studied at the level of individual pixels. The datum $x : \Omega \rightarrow \mathbb{R}$ is in itself a function of a discrete domain $\Omega$, whose elements are called \emph{pixels}. A pixel $u\in\Omega$ is \emph{salient} if changing its intensity $x(u)$ causes $\Phi(x)$ to change significantly, and it is not salient otherwise.

Saliency is usually relative: whether changing $x(u)$ has an impact or not, depends on the values of all the pixels in $x$.\footnote{Defining the saliency of a pixel regardless of the others may be possible, but it would likely be similar to finding the receptive field of the neural network.} Hence saliency is a \emph{local explanation} of a particular prediction performed by the neural network.

The most common way of formalizing the concept of saliency is to linearize $\Phi$ around $x$. Assuming for simplicity the output of the function to be scalar ($d=1$), we can expand it to find:
$$
\Phi(x') \approx \Phi(x) + \langle \nabla \Phi(x), x'-x\rangle.
$$
Each element $w(u)$ of the gradient $w = \nabla \Phi(x)$ can be thought of as the weight of the change $x'(u)-x(u)$ of pixel $u$ in approximating the overall change in the output.
Hence, the gradient can be reshaped in the form of a heat map, interpreted as a \emph{saliency map}.

Note that, while the explanation is local, it is not merely a statement about a specific point $x$; rather, the explanation describes the behavior \emph{around} $x$.
This statement can be made more precise by choosing an accuracy $\epsilon$ for the approximation; then for a sufficiently small neighbourhood $\delta$:
\begin{multline}\label{e:diff}
\forall x' : |x' - x|<\delta\quad\Rightarrow\\
 |\Phi(x') - \Phi(x) - \langle \nabla \Phi(x), x'-x\rangle| < \epsilon.
\end{multline}

The smaller the neighborhood $\delta$, the more limited the explanatory power is.
Generally, explanation methods based on \emph{differential approximations} of the function fail to capture its non-linear lon-range behavior, which is arguably the most interesting and important.
In practice, saliency maps have many limitations, such as being noisy and unable to differentiate neurons when used for studying the response of different units in deep neural networks~\cite{mahendran16salient}.

\paragraph{Extremal perturbations.}

An alternative approach to differential perturbations is to seek for larger perturbations $x'=tx$ of the image with the goal of triggering large changes in the function output.

Formally, given a measure $|t|$ of the size of a perturbation, and assuming that the output is a non-negative scalar, we may seek for the smallest change $t^*$ to the image that causes the output to halve:
\footnote{Alternatively, we can seek for the largest change to the image such that the output is still more than a half:
$$
   t^*=\arg\max_{t\in T} |t|,
   \quad\text{s.t.}\quad
   \Phi(tx) > \frac{1}{2}\Phi(x).
$$}
\begin{equation}\label{e:extremal} 
   t^*=\arg\min_{t\in T} |t|,
   \quad\text{s.t.}\quad
   \Phi(tx) < \frac{1}{2}\Phi(x).
\end{equation}
Such \emph{extremal perturbations} were implicitly adopted by the method of ``meaningful perturbations'' proposed by~\cite{fong17interpretable}.
However, that paper did not characterize formally what kind of information is provided by them, which we do next.

The key is that, while the optimization returns a single \emph{extremal perturbation} $t^*$, the latter implies that \emph{all} smaller changes are insufficient to affect the output significantly (assuming that a global minimizer can be found).
This is thus a statement on a \emph{set} of images:
\begin{equation}\label{e:extremal-motivation}
 \forall t : \quad
 |t| < |t^*| \quad\Rightarrow\quad
 \Phi(tx) \geq \frac{1}{2}\Phi(x).
\end{equation}
We can use this to contrast extremal and differential perturbations: extremal perturbations state something simpler (that the output decreases sufficiently whereas~\cref{e:diff} predicts the actual change) but about a much more diverse class of images (we test $tx$ instead of just neighbors of $x$).

As noted in~\cite{fong17interpretable}, however, it remains important to carefully choose the space of perturbations $T$ and the norm $|t|$.
If insufficient constraints are enforced, the method typically finds tiny adversarial perturbations that trigger idiosyncratic behaviors of the function.
Focusing on more meaningful perturbations allows instead to characterize behaviors that are statistically more relevant to applications.
For attribution, \cite{fong17interpretable}~propose for example to use image blurs as a gentle approximation to removing objects from an image, an approach that we revisit in this paper.

\paragraph{Equivariace to perturbations.}

A limitation of both differential and extremal perturbations is that they describe the representation $\Phi(x)$ around a specific image $x$; they are thus unable to provide global information about the function.
There are several ways of formulating and then testing global hypotheses as well; an example is equivariance, namely the fact that the representation responds in a systematic and predictable manner to particular transformations of the image.
For instance, if $t$ is a mirror flip, $\forall x: \Phi(tx)=\Phi(x)$ means that the representation is invariant (a special case of equivariance) to image flipping;
these and many other properties are for example explored in~\cite{lenc18understanding}.

\subsection{Explanations using privileged information}

So far, the behavior of $\Phi$ has been described based on example inputs $x$ alone.
However, representations are normally learned to capture the \emph{semantic} of data, as may be captured by data labels $y$.
While this privileged information is unavailable to the representation $\Phi(x)$ (usually the goal is to \emph{predict} $y$), it may still be used by the explanation itself.
Formally, we can approximate $\Phi(x)$ using a function of both $x$ and $y$:
\begin{equation}\label{e:exp-priv}
    \Phi(x) \approx e(x,y).
\end{equation}
Note that this is very different from~\cite{wolf18a-formal}
that also consider both images and labels to formulate explanations; in their case $y = \Phi(x)$ is the output of the representation, whereas for us $y$ is the \emph{ground-truth label}.

When the label $y=f(x)$ is  \emph{inferable} form $x$, we may formally substitute $e(x,y) = e(x,\Phi(x)) = \bar e (x)$ in the explanation, reducing it to a function of $x$.
However, this would not be very informative.
Instead, the goal is to devise an interpretable rule $e$ that, given the privileged information $y$, can use it to predict the behaviors of the representation $\Phi(x)$ in a direct and interpretable manner.

\paragraph{Correlation with labels.}

In the simplest example, we may choose as explanation function $e(x,y)=y$, then~\cref{e:exp-priv} states that $\Phi(x)$ is a good predictor for $y$.
However, if the network was trained to predict $y$, this test is analogous to computing the prediction accuracy, so this particular explanation is unlikely to provide novel insights on the function.

A more interesting case is when the privileged information $y$ does not coincide with the labels used to train the representation function $\Phi$ in the first place.
For example, works such as~\cite{bau17network,fong18net2vec} look at the ability of the function to predict auxiliary concepts.
In~\cite{bau17network}, this was done by introducing a new datasets of images  densely labelled with several generic concepts, from texture classes to object parts and materials.
Then the response of individual neurons was correlated to the different classes in a manner similar to testing for a predictor, as suggested above; the difference here is that the spatial location of the neuron response is accounted for when correlation is sought.

\paragraph{Label-induced perturbations.}

We now introduce a new family of explanations.
Assume that $\Phi(x)$ is a classifier trained to recognize a certain object category in image $x$ and let $y(x)$ be the \emph{location} of the object in the image, expressed as a bounding box.
Let $t_y$ a perturbation that depends on the privileged information $y$; for example $t_y$ may blur the box content.
Then we may characterize the behavior of a representation $\Phi(x)$ based on whether blurring the content of such boxes causes the output to change significantly:
\begin{equation}\label{e:privileged}
 \forall x :\quad
 \Phi(t_{y(x)} x) \leq \frac{1}{2} \Phi(x).
\end{equation}
Note the difference between~\cref{e:extremal,e:privileged}.
The first is a statement on the effect of a set of small-enough perturbations applied to a specific image $x$.
The second is a statement on the effect of a single transformation per image, but extended to all possible images.
In the second case, furthermore, the perturbations are entirely predictable form the image label $y$ (the image $x$ is not needed to choose them) and are meaningful ``by design''.

\subsection{Perturbations}

We now define some perturbations $t$. 

\paragraph{Punching holes.}

In the simplest case, $t$ is a mask, namely $tx = t \odot x$ where $t: \Omega \rightarrow \{0,1\}$ or a relaxation of that.
The norm $|t|$ can simply be the complement of the area of the mask.
A regularizer $R(t)$ can be added to constrain the shape of the mask to be regular enough. 

\paragraph{Filling the holes.}

The masking approach can be further refined to induce a blur of the image in the masked are instead of punching a hole~\cite{fong17interpretable}.

Alternatively, one can ``inpaint'' the hole:
$$
tx = \arg\min_{z\in\mathcal{X}} \| t \odot (z - x) \|^2 + Q(z)
$$
where $Q(z)$ is a suitable regularizer such as the norm of the Laplacian:
$$
Q(z) = \int (\nabla^2 z(u))^2 du.
$$

Finally, we consider the \emph{deep image prior} (DP) technique and inpaint as:
$$
tx = \arg\min_{w} \| t \odot (g(w) - x) \|^2
$$
where $g(w)$ is a randomly-initialized generator network with parameters $w$.

\subsection{Learning global explanations}

Next, we look at learning global explanations. Given a network $\Phi$ we can:
\begin{itemize}
\item Learn a generator network $e(x)$ whose goal is to predict an extremal perturbation $t^*$ in the sense discussed before.
\item Learn a scoring function $e(x,t)$ that predicts, for each image $x$ and perturbation $t$, the change $\Phi(tx)-\Phi(x)$.
\item Learn a function $e(t|x)$ that can be interpreted as a probability distribution over transformations $t$. The latter is a variant of the one above. The advantage is that such a distribution may be used to sample transformations for the sake of visualization.
\end{itemize}

Among these, we develop first the second option.
Refining the idea slightly, we may learn a function $e$ that predicts a probability distribution over possible scores after a perturbation has been applied:
$$
    e(x,t,\Phi(x)) = p(\Phi(tx)|x,t).
$$
Note that $\Phi(tx)$ can be calculated deterministically, so one may wonder why this is meaningful.
There main reason is that $e$ provides a compact summary of what may be learned from such perturbations.
In particular:
\begin{itemize}
\item We can make $e$ a simple model, so that evaluating it for different $t$ is very fast. This allows us to quickly plot heatmaps as functions of $t$.
\item Globally, we can learn $e$ much faster than computing all perturbations $\Phi(tx)$ for all images $x$ in the training set. In fact, for each image we may sample at random just a couple of transformations to train $e$ from.
\item Note also that we use a probabilistic formulation since $e$ is only a fast approximation of the effect of applying the perturbation of the network, so it may be off.
\end{itemize}

\paragraph{With privileged information.}

Assume that we have learned $e(x,t,\Phi(x))$ as explained above.
We can learn two more explanation functions:
\begin{itemize}
\item A function $e(x,y,t,\Phi(x))$ that depends \emph{also} on the privileged information $y$. This can be simpler than $e(x,t,\Phi(x))$.
\item A function $e(y,t,\Phi(x))$ that \emph{only} uses $y$ but not $x$.
\end{itemize}
The latter is particularly interesting as it allows us to answer the question on whether the effect of perturbations is completely predicted by the semantic content of the image (i.e. $y$ is a sufficient statistics for predicting the perturbation effect) or whether $x$ is also needed.
The latter can be quantified by comparing the accuracy of predictors $e(x,y,t,\Phi(x))$ and $e(y,t,\Phi(x))$.


\subsection{Inverting explanation}

Suppose we have found out that intermediate neurons $m$ are salient. Then we solve the reconstruction problem:
$$
\min_{x}
$$


\begin{table*}
\begin{tabular}{r|c|c|c|c|c|l|}
\cline{2-7}
                                & \multicolumn{3}{c|}{\textbf{VOC07 Test (All/Diff)}}                                        & \multicolumn{3}{c|}{\textbf{COCO14 Val (All/Diff)}}                                                 \\ \hline
\multicolumn{1}{|r|}{} & \textit{VGG16}             & \textit{GoogLeNet}             & \textit{ResNet50}             & \textit{VGG16}             & \textit{GoogLeNet}             & \multicolumn{1}{c|}{\textit{ResNet50}} \\ \hline
\multicolumn{1}{|r|}{\textbf{Gradient}} &76.3\% / 59.9\%&                       &                       &                       &                       &                                \\ \hline
\multicolumn{1}{|r|}{\textbf{Guided Backprop}} &73.1\% / 53.6\% &                       &                       &                       &                       &                                \\ \hline
\multicolumn{1}{|r|}{\textbf{LRP*}} &--&                       &                       &                       &                       &                                \\ \hline
\multicolumn{1}{|r|}{\textbf{CAM}} &--&                       &                       &                       &                       &                                \\ \hline
\multicolumn{1}{|r|}{\textbf{Grad-CAM}} &79.0\% / 64.3\%&                       &                       &                       &                       &                                \\ \hline
\multicolumn{1}{|r|}{\textbf{EB*}} &76.9\% / 55.1\%&                       &                       &                       &                       &                                \\ \hline
\multicolumn{1}{|r|}{\textbf{Contrast EB*}} &80.0\% / 66.8\%&                       &                       &                       &                       &                                \\ \hline
\multicolumn{1}{|r|}{\textbf{RISE}}  &\textbf{82.7\%}/\textbf{77.19\%}&                       &                       &                       &                       &                                \\ \hline
\multicolumn{1}{|r|}{\textbf{Ours (Mask)}} &\textbf{85.5\%} / \textit{\textbf{76.8\%}}&  & &  & &\\ \hline
\end{tabular}
\begin{caption}Pointing Precision. *copied from ~\cite{zhang2016excitation}. **copied from ~\cite{X}.\end{caption}
\end{table*}
\subsubsection{Average Precision}
We also evaluate the quality of various visual attribution methods using average precision. Each visualization is used to generate a ranked order of the importance of pixels.

\begin{table*}
\begin{tabular}{r|c|c|c|c|c|l|}
\cline{2-7}
                                & \multicolumn{3}{c|}{\textbf{VOC07 Test (All/Diff)}}                                        & \multicolumn{3}{c|}{\textbf{COCO14 Val (All/Diff)}}                                                 \\ \hline
\multicolumn{1}{|r|}{} & \textit{VGG16}             & \textit{GoogLeNet}             & \textit{ResNet50}             & \textit{VGG16}             & \textit{GoogLeNet}             & \multicolumn{1}{c|}{\textit{ResNet50}} \\ \hline
\multicolumn{1}{|r|}{\textbf{Gradient}} &60.4\% / 42.5\%&                       &                       &                       &                       &                                \\ \hline
\multicolumn{1}{|r|}{\textbf{Guided Backprop}} &63.0\% / 42.3\% &                       &                       &                       &                       &                                \\ \hline
\multicolumn{1}{|r|}{\textbf{CAM}} &--&                       &                       &                       &                       &                                \\ \hline
\multicolumn{1}{|r|}{\textbf{Grad-CAM}} &63.8\%/46.2\% &                       &                       &                       &                       &                                \\ \hline
\multicolumn{1}{|r|}{\textbf{RISE}}  &\textit{\textbf{64.0\%}} / \textit{\textbf{52.8\%}}&                       &                       &                       &                       &                                \\ \hline
\multicolumn{1}{|r|}{\textbf{Ours (Mask)}} &\textbf{67.5\%} / \textbf{52.9\%}&  & &  & &\\ \hline
\end{tabular}
\begin{caption}Average Precision.\end{caption}
\end{table*}

\subsection{Investing Architectures}
We generate masks on the following architectures pre-trained on ImageNet:
\begin{enumerate}
    \item AlexNet
    \item VGG16
    \item GoogLeNet
    \item ResNet50
\end{enumerate}
\todo{Need to decide how to evaluate/analyze this -- test for area coverage}
\todo{Generate masks on ImageNet val for AlexNet, VGG16, GoogLeNet, and ResNet50}



==> tbl-imagenet.tex <==
\begin{table}
\centering
\setlength{\tabcolsep}{2pt}
\begin{tabular}{lccccccc}
\toprule
       & \multicolumn{1}{c}{\emph{Avg. Prec}}  & \multicolumn{6}{c}{\emph{BBox Localization}} \\
Method & AP & Mea-\textit{$\alpha$} & \textit{E(\%)} & Min-\textit{$\alpha$} & \textit{E(\%)} & Ene-\textit{$\alpha$} & \textit{E(\%)}    \\
\midrule
Grad   & 78.3  & 1.5  & 46.4 & 0.2  & 47.5 & 0.45  & 46.7\\
Guid  & $\bm{81.8}$  & 2.0  & $\bm{40.0}$ & 0.05  & 49.5 & 0.6  & $\bm{40.3}$ \\
G-Cam & 47.7  & 2.0  & 58.1 & 0.3  & 59.0 & 0.4  & 58.9\\
RISE   & 63.9  & 1.0 & 59.3 & 0.65  & 54.1 & 0.1  & 54.9 \\ 
Ours   & 75.7  & 1.0  & 48.0 & 0.5  & $\bm{45.4}$ & 0.55  & 45.1\\
\bottomrule
\end{tabular}
\caption{\textbf{Weakly Supervised Localization.} Average Precision and Bounding Box Localization Error on ImageNet validation set for different attribution methods. 
}\label{tbl:imagenet_loc}
\end{table}

==> tbl-monotonic.tex <==
\begin{table}[]
\begin{tabular}{rcc}
                                & \textbf{Preservation} & \textbf{Deletion} \\ \cline{2-3} 
\multicolumn{1}{r|}{\textbf{Average Monotonicity}} &73.21\% & 44.24\%
\end{tabular}
\caption{\textbf{Monotonicity.} This table reports average monotocity of the area curve graphs for preservation and deletion (\cref{fig:area_growing}a) when optimized for using the preservation loss $N\approx 10k$ in the ImageNet validation set. An area curve is considered monotonic if its target logits scores are non-decreasing or non-increasing for preservation and deletion respectively.}\label{tbl:monotonic}
\end{table}
